Finding Rule-Interpretable Non-Negative Data Representation

Non-negative Matrix Factorization (NMF) is an intensively used technique for obtaining parts-based, lower dimensional and non-negative representation. Researchers in biology, medicine, pharmacy and other fields often prefer NMF over other dimensionality reduction approaches (such as PCA) because the non-negativity of the approach naturally fits the characteristics of the domain problem and its results are easier to analyze and understand. Despite these advantages, obtaining exact characterization and interpretation of the NMF's latent factors can still be difficult due to their numerical nature. Rule-based approaches, such as rule mining, conceptual clustering, subgroup discovery and redescription mining, are often considered more interpretable but lack lower-dimensional representation of the data. We present a version of the NMF approach that merges rule-based descriptions with advantages of part-based representation offered by the NMF. Given the numerical input data with non-negative entries and a set of rules with high entity coverage, the approach creates the lower-dimensional non-negative representation of the input data in such a way that its factors are described by the appropriate subset of the input rules. In addition to revealing important attributes for latent factors, their interaction and value ranges, this approach allows performing focused embedding potentially using multiple overlapping target labels.

==> table_datasets.tex <==
\begin{tabular}{@{}
  l% name
  l% code
  S[table-format=5.0,group-minimum-digits=4]% rows
  S[table-format=5.0,group-minimum-digits=4]% columns
  S[table-format=1.0]% classes
  r% reference
  @{}}
  \toprule
  name & code & {\#row} & {\#col} & {\#class} & ref.  \\
  \midrule
  Abalone & AB & 4177 & 7 &  2 & \cite{KaggleAbalone}\\
  Arrhythmia & AR & 452  & 106  & 2 &  \cite{Dua2019UCIML} \\
  Brain cancer & BRC & 130 & 54676 &  5 & \cite{KaggleBrainCancer} \\
  Nomao & NM & 34465 & 89 & 2 &  \cite{NOMAO}\\
  \ifappendix
  Parkinson's disease& PD & 252  & 457 &  2 & \cite{sakar2019comparative}\\
  Secom & SE & 1567 & 438 &  2 & \cite{Dua2019UCIML}\\
  \fi
  Sports articles & SA & 1000 & 57 &  2 &   \cite{hajj2019subjectivity}\\
  \ifappendix
   Heart disease & HD & 4238 & 15 & 2 &  \cite{Dua2019UCIML}\\
  Leukemia & LK & 64 & 22284 & 5 &  \cite{KaggleLeukemia}\\
  Breast cancer & BC & 569 & 30 &  2 & \cite{Dua2019UCIML} \\
  Wine & WN & 178 & 12 &   3 & \cite{Dua2019UCIML} \\
  \fi
  $4$News & $4$N & 400 & 800 &  {--} &\cite{MiettinenPhD}\\
  Gene functions & BO & 3475 & 4523 &  {--} &\cite{MihelcicBio}\\
  \ifappendix
  Bacterial phenotypes  & PH & 92 & 1230 &  {--} &\cite{Brbic}\\
  \fi
 World Countries& WC & 141 & 328 &  {--} &\cite{Trade}\\
  \bottomrule
\end{tabular}

==> table_results_descriptive.tex <==
\begin{tabular}{@{}
  l% Data
  S[table-format=2.0]% k
  S[table-format=5.1,group-minimum-digits=4]% #iters
  S[table-format=2.2]% RE
  S[table-format=3.2]% DE
  S[table-format=+1.2]% ACD
  L% Algorithm
  @{}}
  \toprule
  {$\mathcal{D}$} & {$k$} & {\#iters} & {$\mathit{RE}$}  &  {$\mathit{DE}$} & {$\mathit{ADC}$} & \text{algorithm}  \\
  \midrule
AB & 5 & 3357.4 &3.70  & 54.00 & 0.00 & \DNMF{ind} \\
 & & 1746.2 & 3.66 & 43.46 & -0.11 & \DNMF{indA}\\
& & 4419.0 & 3.67 & \bfseries 36.08 &  -0.14 & \DNMF{dir} \\
 & & 2145.9 & 3.32 & 36.81 & \bfseries -0.16 & \DNMF{dirA}\\
 & & 3685.3 & 3.87 & 54.42 & -0.00 & \DNMF{comb}\\
 & & 15396.0 & \bfseries 1.93  & 101.28  & 0.19 & \NMF{MU} \\
  & & 138.9 & 19.05 & 103.71 & 0.42 & \NMF{sp} \\
  & & 834.0 & 21.62 & 88.17 & 0.15 & \NMF{bf} \\[.7ex]  %\hline 
  AR & 20 & 15227.0 & 19.99 & 60.00  & 0.00 &\DNMF{ind} \\
   & & 13453.0 & 19.81 & 58.84 & 0.00 & \DNMF{indA}\\
 & & 5623.0 & 20.07 & \bfseries 16.71 &  \bfseries -0.28 & \DNMF{dir} \\
   & & 11118.8 & 20.54 & 20.15 & -0.28 & \DNMF{dirA}\\
    & & 13995.0 & 20.26 & 59.60 & -0.01 & \DNMF{comb}\\
  & & 22437.0 & \bfseries 11.16 & 98.10 & 0.48 & \NMF{MU}\\
 & & 50000.0 & 12.00  & 97.76  & 0.45 & \NMF{sp}\\
  & & 21.0 & 20.45  & 92.41  & 0.27 & \NMF{bf}\\[.7ex] %\hline
   BRC & 40 & 9482.2 & 5.88  & 13.08 & 0.00  & \DNMF{ind} \\
    & & 9999.0 & 5.56 & 16.51 & 0.06 & \DNMF{indA}\\
  & & 9999.0 & 6.09  & 7.61  &  0.01  & \DNMF{dir} \\
  & & 9999.0 & 4.02 & 80.80 & 0.75 & \DNMF{dirA}\\
  & & 9543.8 & 6.53 & \bfseries 7.21 & \bfseries -0.01 & \DNMF{comb}\\
 & & 9999.0 & \bfseries 3.96  & 112.08  & 0.91  & \NMF{MU} \\
 & & 10000.0 & 4.08 & 108.64 & 0.93& \NMF{sp}\\
  & & 2.0 & 62.59 & 146.00 & 0.81 & \NMF{bf} \\[.7ex]  %\hline
   NM & 40 & 9999.0 & 17.11 & 75.53  & 0.00 &\DNMF{ind}  \\
    & & 9999.0 & 15.21 & 74.83 & -0.01 & \DNMF{indA}\\
  & & 5486.0 & 11.03 & \bfseries 12.49 &  \bfseries -0.55 & \DNMF{dir} \\
    & & 3682.0 & 12.18 & 12.93 & -0.55 & \DNMF{dirA}\\
     & & 9999.0 & 18.05 & 74.36 & -0.02 & \DNMF{comb}\\
 & & 9999.0 & \bfseries 2.52 & 88.72 & 0.18 & \NMF{MU} \\
 & & 10000.0 & 3.75 & 73.96 & -0.07 & \NMF{sp} \\
  & & 860.0 & 42.21 & 78.65 & 0.01 & \NMF{bf} \\[.7ex]
  \ifappendix %% BEGIN if appendix
   PD & 40 & 20645.6 &  1.07 & 63.21 & 0.00 &\NMF{D} \\
  & & 49999.0 & 0.29 & 22.13 &  -0.28 & \NMF{DE} \\
 & & 30600.0 & 0.13 & 128.82  & 0.52 & \NMF{MU} \\
  & & 2.0 & 27.51 & 153.82 & 0.46 & \NMF{sp}\\
  & & 5.0 & 57.00 & 146.49 & 0.30 & \NMF{bf}\\[.7ex] %\hline
 SE & 60 & 17702.8 & 6.07 & 87.90 & 0.00 &\NMF{D} \\
 & & 12760.2 & 3.06 & 52.76 &  -0.34 & \NMF{DE} \\
  & & 49999.0 & 0.84 & 115.38 & 0.21  & \NMF{MU} \\
 & & 50000.0 & 3.39 & 110.26 & 0.22 & \NMF{sp}\\
 & & 25.0 & 58.53 & 160.89 & 0.12 & \NMF{bf}\\[.7ex] %\hline
  \fi %% END if appendix
  SA & 20 & 10663.0 & 5.42 & 70.71  & 0.00 &\DNMF{ind} \\
   & & 17545.0 & 4.51 & 66.70 & -0.06 & \DNMF{indA}\\
  & & 18965.8 & 5.35 & \bfseries 18.12 &  \bfseries -0.43 & \DNMF{dir} \\
  & & 14102.7 & 4.74 & 25.63 & -0.35 & \DNMF{dirA}\\
  & & 9402.0 & 6.07 & 70.21 & -0.01 & \DNMF{comb}\\
  & & 46318.8 & \bfseries 1.68 & 119.02 & 0.36 & \NMF{MU}\\
  & & 50000.0 &  2.57 & 110.75 & 0.43 & \NMF{sp}\\
  & & 49.0 &  29.24 & 128.66 & 0.39 & \NMF{bf}\\[.7ex] %\hline
  \ifappendix %% BEGIN if appendix
    LK & 15 & 9999.0 & 3.09  & 81.00 & 0.00  & \DNMF{ind} \\
    & & 9999.0 & 3.10 & 78.00 & -0.01 & \DNMF{indA}\\
  & & 9999.0 & 3.05  & 82.83  &  -0.03  & \DNMF{dir} \\
  & & 9999.0 & 2.99 & 108.72 & 0.09 & \DNMF{dirA}\\
  & & 9999.0 & 3.28 & 62.88 & -0.20 & \DNMF{comb}\\
 & & 9999.0 & 2.97  & 141.00  & 0.28  & \NMF{MU} \\
 & & 10000.0 & 3.67 & 113.12 & 0.36& \NMF{sp}\\
  & & 3.0 & 4.58 & 166.24 & 0.26 & \NMF{bf} \\[.7ex]  %\hline
  BC & 8 & 2671.0 & 8.97 &  64.09 & 0.00 & \NMF{D}\\
  & & 3684.6  & 7.05 & 38.60 &  -0.32 & \NMF{DE} \\
 & & 30085.2 & 0.19 & 103.05 & 0.32 & \NMF{MU}\\
 & & 50000.0 &  0.58 & 103.54  & 0.46 & \NMF{sp} \\
 & & 70.0 &  24.46 & 102.59  & 0.27 & \NMF{sp} \\[.7ex] %\hline
 HD & 8 & 9791.0 & 7.51 & 71.47  & 0.00 &\DNMF{ind}  \\
    & & 13158.0 & 5.95 & 72.95 & 0.03 & \DNMF{indA}\\
  & & 7390.4 & 7.10 & 35.40 &  -0.31 & \DNMF{dir} \\
     & & 12052.3 & 6.62 & 29.15 & -0.32 & \DNMF{dirA}\\
      & & 12721.0 & 6.98 & 71.37 & -0.01 & \DNMF{comb}\\
 & & 33855.8 & 0.42 & 107.62 & 0.21 & \NMF{MU} \\
  & & 27371.4 & 13.57 & 104.04 & 0.39& \NMF{sp} \\
  & & 528.0 & 14.28 & 113.75 & 0.28& \NMF{bf} \\[.7ex] %\hline
 WN & 8 & 8768.0 & 4.46 & 10.12 & 0.00 &\NMF{D} \\
 & & 11002.0 & 4.17 & 9.73 &  0.00 & \NMF{DE} \\
   & & 49931.2 & 0.43 & 84.50 & 0.62 & \NMF{MU}\\
   &  & 50000.0 & 0.41 &  84.68 & 0.63 & \NMF{sp} \\
 &  & 21.0 & 10.76 &  86.81 & 0.60 & \NMF{sp} \\[.7ex] %\hline
  \fi %% END if appendix
  4N & 60 & 1500.0 & 50.55 & 64.40 & 0.00 &\DNMF{ind} \\
   & & 1023.0 & 47.57 & 62.92 & 0.04 & \DNMF{indA}\\
  & & 1193.2 & 50.00 & 43.32 &  -0.12 & \DNMF{dir} \\
  & & 1221.6 & 49.88 & \bfseries 41.14 & \bfseries -0.15 & \DNMF{dirA}\\
  & & 3963.0 & 50.56 & 64.73 & 0.00 & \DNMF{comb}\\
 & & 1089.0 & \bfseries 37.22 & 114.15 & 0.53 & \NMF{MU}\\
 & & 34277.9 & 41.64 & 121.17  & 0.53 & \NMF{sp}\\
  & & 5.0 & 67.74 & 267.12  & 0.47 & \NMF{bf}\\
  \bottomrule
\end{tabular}

==> table_results_jaccard.tex <==
\begin{tabular}{@{}
  l% data
  r% avgJ_sup
  r% avgJ_desc
  l% algorithm 
  @{}}
  \toprule
  $\mathcal{D}$ & $\xbar{\mathit{jacc}}_{\text{supp}}$ & $\xbar{\mathit{jacc}}_{\text{desc}}$ & algorithm  \\
  \midrule
AB & $0.38$ & $\mathbf{0.78}$ & $\NMF{D}$  \\
  & $\mathbf{0.42}$ &  $\mathbf{0.78}$ & $\NMF{DE}$ \\
  &  $0.20$ &  $0.26$ & $\NMF{MU}$ \\
  &  $0.23$ &  $0.16$ & $\NMF{sp}$ \\[.7ex] %\hline
   AR & $0.48$ & $0.67$ & $\NMF{D}$ \\
 &  $\mathbf{0.76}$ &  $\mathbf{0.90}$ & $\NMF{DE}$ \\
  &  $0.11$ & $0.16$ & $\NMF{MU}$\\
 &  $0.05$ & $0.21$ & $\NMF{sp}$\\[.7ex]  %\hline
    HD & $0.42$ & $0.53$ & $\NMF{D}$ \\
  & $\mathbf{0.52}$ &  $\mathbf{0.80}$ & $\NMF{DE}$ \\
 &  $0.23$  & $0.39$ & $\NMF{MU}$ \\
  & $0.11$  & $0.15$ & $\NMF{sp}$\\[.7ex]  %\hline
   NM & $0.47$  & $0.30$  & $\NMF{D}$ \\
  &  $\mathbf{0.77}$  &  $\mathbf{0.94}$  & $\NMF{DE}$ \\
 & $0.09$  & $0.25$  & $\NMF{MU}$ \\
  &  $0.03$ & $0.12$& $\NMF{sp}$\\[.7ex] 
    PD & $0.52$  & $0.62$ & $\NMF{D}$ \\
  & $\mathbf{0.67}$ &  $\mathbf{0.90}$ & $\NMF{DE}$ \\
 &  $0.19$ & $0.09$ & $\NMF{MU}$ \\
  &  $0.13$ & $0.13$ & $\NMF{sp}$ \\[.7ex]  %\hline
  SE & $0.32$  &$0.26$ & $\NMF{D}$ \\
 & $\mathbf{0.64}$ &  $\mathbf{0.59}$ & $\NMF{DE}$ \\
  & $0.10$  & $0.05$  &  $\NMF{MU}$\\
 &  $0.09$  & $0.04$  & $\NMF{sp}$ \\[.7ex]  %\hline
  SA  & $0.42$ & $0.47$ & $\NMF{D}$ \\
  & $\mathbf{0.85}$ &  $\mathbf{0.76}$ & $\NMF{DE}$ \\
  & $0.11$ & $0.10$ & $\NMF{MU}$ \\
 & $0.07$ &$0.06$ & $\NMF{sp}$  \\[.7ex]  %\hline
  BC & $0.49$ & $0.61$ & $\NMF{D}$ \\
  & $\mathbf{0.85}$ &  $\mathbf{0.91}$ & $\NMF{DE}$ \\
 & $0.17$ & $0.29$  & $\NMF{MU}$ \\
  &  $0.08$ & $0.11$ & $\NMF{sp}$ \\[.7ex]  %\hline
  WN & $0.62$ & $\mathbf{1.00}$ & $\NMF{D}$ \\
 & $\mathbf{0.83}$ &  $\mathbf{1.00}$ & $\NMF{DE}$ \\
  & $0.32$ & $0.37$ &  $\NMF{MU}$\\
                &  $0.13$  & $0.37$ & $\NMF{sp}$ \\[.7ex]  %\hline
  4N & -- & $0.70$ & $\NMF{D}$ \\
 & -- &  $\mathbf{0.75}$ & $\NMF{DE}$ \\
  & -- & $0.02$ &  $\NMF{MU}$\\
                &  --  & $0.03$ & $\NMF{sp}$ \\
  \bottomrule
 \end{tabular} 

==> table_results_redescriptions.tex <==
\begin{tabular}{@{}
  l% Data
  S[table-format=2.0]% k
  S[table-format=5.1,group-minimum-digits=4]% #iters
  S[table-format=2.2]% RE
  S[table-format=3.2]% DE
  S[table-format=+1.2]% ACD
  L% Algorithm
  @{}}
  \toprule
  {$\mathcal{D}$} & {$k$} & {\#iters} & {$\mathit{RE}$}  &  {$\mathit{DE}$} & {$\mathit{ADC}$} & \text{algorithm}  \\
  \midrule
AB & 5 & 8647.0 & 3.68  & 46.17 & 0.00 & \DNMF{ind} \\
 & & 9733.0 & 3.87 & 51.18 & 0.06 & \DNMF{indA}\\
& & 1353.0 & 3.43 & 47.02 &  0.04 & \DNMF{dir} \\
& & 1746.5 & 3.63 & \bfseries 39.51 & 0.03 & \DNMF{dirA}\\
& & 12440.0 & 3.48 & 46.22 & \bfseries -0.00 & \DNMF{comb}\\
 & & 14553.0 & \bfseries 1.94  & 104.90  & 0.43 & \NMF{MU} \\
  & & 13941.0 & 9.83 & 98.55 & 0.58 & \NMF{sp} \\
  & & 834.0 & 21.62 & 99.58 & 0.42 & \NMF{bf} \\[.7ex]  %\hline
  AR & 10 & 1516.2 & 20.31 & 65.53  & 0.00 &\DNMF{ind} \\
   & & 11726.6 & 19.56 & 66.99 & 0.03 & \DNMF{indA}\\
 & & 4092.0 & 19.73 & \bfseries 31.34 &  \bfseries -0.18 & \DNMF{dir} \\
 & & 18975.1 & 18.68 & 37.48 & -0.05 & \DNMF{dirA}\\
 & & 1245.4 & 20.90 & 64.32 & -0.01 & \DNMF{comb}\\
  & & 12666.0 & \bfseries 15.48 & 115.25 & 0.43 & \NMF{MU}\\
 & & 34390.8 & 19.00  & 106.59  & 0.51 & \NMF{sp}\\
  & & 44.0 & 22.04  & 117.48  & 0.32 & \NMF{bf}\\[.7ex] %\hline
  BRC & 50 & 9999.0 & 5.80  & 9.43 & 0.00  & \DNMF{ind} \\
    & & 9999.0 & 5.79 & 5.61 & -0.01 & \DNMF{indA}\\
  & & 5719.0 & 6.24  & \bfseries 0.00  & \bfseries -0.01  & \DNMF{dir} \\
  & & 9999.0 & 3.69 & 55.47 & 0.69 & \DNMF{dirA}\\
  & & 9999.0 & 6.26 & 9.40 & 0.00 & \DNMF{comb}\\
 & & 9999.0 & 3.57  & 102.60  & 0.92  & \NMF{MU} \\
 & & 10000.0 & \bfseries 3.56 & 102.86 & 0.92& \NMF{sp}\\
  & & 1.0 & 63.86 & 111.94 & 0.74 & \NMF{bf} \\[.7ex]  %\hline
   NM & 10 & 9999.0 & 11.59 & 56.52  & 0.00 &\DNMF{ind}  \\
    & & 9250.6 & 9.06 & 58.80 & 0.12 & \DNMF{indA}\\
  & & 3650.0 & 10.55 & \bfseries 23.20 &  \bfseries -0.28 & \DNMF{dir} \\
  & & 7480.4 & 9.09 & 32.35 & -0.05 & \DNMF{dirA}\\
   & & 9999.0 & 10.98 & 56.02 & -0.00 & \DNMF{comb}\\
 & & 9999.0 & \bfseries 5.08 & 102.10 & 0.36 & \NMF{MU} \\
 & & 10000 & 7.10 & 101.15 & 0.49 & \NMF{sp} \\
  & & 3445.0 & 16.24 & 106.71 & 0.38 & \NMF{bf} \\[.7ex]
  \ifappendix %% BEGIN if appendix
   PD & 10 & 25023.0 &  1.02 & 58.87 & 0.00 &\NMF{D} \\
  & & 47052.4 & 1.07 & 28.92 &  -0.23 & \NMF{DE} \\
 & & 43808.0 & 0.29 & 105.58  & 0.40 & \NMF{MU} \\
  & & 2.1 & 21.64 & 110.60 & 0.31 & \NMF{sp}\\
  & & 24.0 & 26.30 & 99.90 & 0.31 & \NMF{bf}\\[.7ex] %\hline
 SE & 10 & 6020.0 & 10.91 & 84.63 & 0.00 &\NMF{D} \\
 & & 22290.8 & 10.88 & 52.01 &  -0.38 & \NMF{DE} \\
  & & 14778.0 & 7.43 & 105.50 & 0.18  & \NMF{MU} \\
 & & 50000.0 & 9.16 & 103.02 & 0.20 & \NMF{sp}\\
  & & 155.0 & 29.13 & 110.32 & 0.08 & \NMF{bf}\\[.7ex] %\hline
  \fi %% END if appendix
  SA & 10 & 12428.0 & 4.78 & 69.25  & 0.00 &\DNMF{ind} \\
   & & 19560.0 & 3.90 & 65.83 & 0.02 & \DNMF{indA}\\
  & & 16321.9 & 4.86 & \bfseries 29.79 &  \bfseries -0.37 & \DNMF{dir} \\
   & & 26522.4 & 4.32 & 29.84 & -0.26 & \DNMF{dirA}\\
   & & 15823.0 & 4.83 & 69.14 & -0.00 & \DNMF{comb}\\
  & & 28184.8 & \bfseries 3.01 & 106.58 & 0.31 & \NMF{MU}\\
 & & 50000.0 &  3.51 & 103.73 & 0.35 & \NMF{sp}\\
  & & 99.0 &  33.42 & 106.11 & 0.29 & \NMF{bf}\\[.7ex] %\hline
  \ifappendix %% BEGIN if appendix
      LK & 50 & 5402.0 & 3.29  & 0.00 & 0.00  & \DNMF{ind} \\
    & & 7567.0 & 3.15 & 0.00 & 0.00 & \DNMF{indA}\\
  & & 9999.0 & 2.37  & 0.00  &  0.00  & \DNMF{dir} \\
  & & 9999.0 & 1.47 & 12.32 & 0.03 & \DNMF{dirA}\\
  & & 2944.0 & 3.78 & 0.00 & 0.00 & \DNMF{comb}\\
 & & 9999.0 & 1.17  & 112.69  & 0.89  & \NMF{MU} \\
 & & 10000.0 & 1.10 & 109.52 & 0.92& \NMF{sp}\\
  & & 1.0 & 75.49 & 146.16 & 0.76 & \NMF{bf} \\[.7ex]  %\hline
  BC & 8 & 3252.0 & 8.04 &  64.07 & 0.00 & \NMF{D}\\
  & & 1821.0  & 8.18 & 24.21 &  -0.36 & \NMF{DE} \\
 & & 24238.4 & 0.21 & 97.12 & 0.28 & \NMF{MU}\\
  & & 50000.0 &  0.34 & 102.98  & 0.45 & \NMF{sp} \\
  & & 70.0 &  24.46 & 98.52  & 0.24 & \NMF{bf} \\[.7ex] %\hline
   HD & 8 & 23051.0 & 5.95 & 68.44  & 0.00 &\DNMF{ind}  \\
    & & 19235.0 & 5.54 & 67.56 & -0.01 & \DNMF{indA}\\
  & & 11175.0 & 5.80 & 23.72 &  -0.39 & \DNMF{dir} \\
  & & 14099.8 & 5.96 & 21.59 & -0.41 & \DNMF{dirA}\\
  & & 21310.0 & 5.54 & 67.79 & -0.01 & \DNMF{comb}\\
   & & 32854.0 & 0.42 & 94.92 & 0.17& \NMF{MU} \\
 & & 40000.8 & 7.25 & 97.90 & 0.30 & \NMF{sp} \\
  & & 528.0 & 14.28 & 90.86 & 0.18& \NMF{bf} \\[.7ex]
   %\hline
 WN & 8 & 15358.0 & 3.73 & 61.27 & 0.00 &\NMF{D} \\
 & & 21560.0 & 3.61 & 8.35 &  -0.35 & \NMF{DE} \\
   & & 49462.2 & 0.42 & 100.50 & 0.37 & \NMF{MU}\\
   &  & 50000.0 & 0.72 &  97.16 & 0.40 & \NMF{sp} \\
 &  & 21.0& 10.76 &  82.89 & 0.13 & \NMF{bf} \\[.7ex] %\hline
  \fi %% END if appendix
  4N & 60 & 1531.0 & 52.27 & 86.41 & 0.00 &\DNMF{ind} \\
   & & 2461.0 & 51.74 & 76.41 & -0.07 & \DNMF{indA}\\
  & & 1171.7 & 51.50 & 47.94 &  -0.35 & \DNMF{dir} \\
  & & 994.4 & 51.61 & \bfseries 46.50 & \bfseries -0.36 & \DNMF{dirA}\\
  & & 1969.0 & 53.85 & 83.96 & -0.04 & \DNMF{comb}\\
 & & 1445.0 & \bfseries 37.12 & 111.30 & 0.27 & \NMF{MU}\\
& & 37727.6 & 41.25 & 116.25  & 0.27 & \NMF{sp}\\
& & 5.0 & 67.74 & 237.56  & 0.20 & \NMF{bf}\\[.7ex]
WC & 20 & 31800.6 & 0.75 & 54.26 & 0.00 &\DNMF{ind} \\
 & & 30194.6 & 0.80 & 51.40 & 0.00 & \DNMF{indA}\\
  & & 39822.8 & 1.06 & 49.81 &  \bfseries -0.05 & \DNMF{dir} \\
  & & 49999.0 & 1.24 & \bfseries 43.48 & -0.03 & \DNMF{dirA}\\
  & & 13011.0 & 1.12 & 52.89 & -0.02 & \DNMF{comb}\\
 & & 5085.0 & \bfseries 0.61 & 118.37 & 0.66 & \NMF{MU}\\
& & 15307.2 & 31.23 & 163.32  & 0.45 & \NMF{sp}\\
& & 6.0 & 4.40 & 109.05  & 0.67 & \NMF{bf}\\[.7ex]
\ifappendix %% BEGIN if appendix
PH & 30 & 186.2 & 58.20 & 61.07 & 0.00 &\NMF{D} \\
  & & 212.2 & 63.10 & 38.25 &  -0.19 & \NMF{DE} \\
 & & 139.0 & 35.75 & 102.98 & 0.46 & \NMF{MU}\\
& & 12794 & 40.96 & 110.30  & 0.40 & \NMF{sp}\\
& & 2.0 & 44.87 & 110.45  & 0.38 & \NMF{bf}\\[.7ex]
\fi
BO & 30 & 49999.0 & 5.68 & 71.34 & 0.00 &\DNMF{ind} \\
 & & 49999.0 & 5.54 & 65.94 & 0.22 & \DNMF{indA}\\
  & & 43196.0 & 6.10 & 14.15 &  \bfseries -0.32 & \DNMF{dir} \\
  & & 49999.0 & 5.83 & \bfseries 13.77 & -0.12 & \DNMF{dirA}\\
  & & 49999.0 & 5.89 & 72.07 & -0.10 & \DNMF{comb}\\
 & & 16694.0 & \bfseries 5.45 & 184.66 & 0.36 & \NMF{MU}\\
& & 338.6 & 28.58 & 112.21  & 0.39 & \NMF{sp}\\
& & 114.0 & 6.99 & 211.77  & 0.34 & \NMF{bf}\\
  \bottomrule
\end{tabular}

==> table_results_subgroups.tex <==
\begin{tabular}{@{}
  l% Data
  S[table-format=2.0]% k
  S[table-format=5.1,group-minimum-digits=4]% #iters
  S[table-format=2.2]% RE
  S[table-format=3.2]% DE
  S[table-format=+1.2]% ACD
  L% Algorithm
  @{}}
  \toprule
  {$\mathcal{D}$} & {$k$} & {\#iters} & {$\mathit{RE}$}  &  {$\mathit{DE}$} & {$\mathit{ADC}$} & \text{algorithm}  \\
  \midrule
%\hline
  AR & 20 & 2833.0 & 24.65 & 65.39  & 0.00 &\DNMF{ind} \\
   & & 3606.0 & 24.61 & 65.54 & 0.00 & \DNMF{indA}\\
 & & 12685.0 & 25.46 & \bfseries 2.70 &  \bfseries -0.43 & \DNMF{dir} \\
 & & 49999.0 & 25.64 & 3.54 & -0.43 & \DNMF{dirA}\\
 & & 13479.3 & 24.51 & 65.54 & 0.00 & \DNMF{comb}\\
  & & 6610.0 & \bfseries 20.24 & 72.49 & 0.10 & \NMF{MU}\\
 & & 26119.6 & 21.80  & 21.51  & -0.38 & \NMF{sp}\\
 & & 89.0 & 23.93  & 70.57  & 0.06 & \NMF{bf}\\[.7ex] %\hline
     BRC & 25 & 7658.6 & 6.03  & 29.94 & 0.00  & \DNMF{ind} \\
    & & 8377.2 & 5.64 & 31.38 & 0.02 & \DNMF{indA}\\
  & & 9999.0 & 5.08  & 47.71  &  0.17  & \DNMF{dir} \\
  & & 9999.0 & 4.74 & 86.65 & 0.53 & \DNMF{dirA}\\
  & & 2684.0 & 6.82 & \bfseries 21.29 & \bfseries -0.04 & \DNMF{comb}\\
 & & 9999.0 & \bfseries 4.69  & 111.12  & 0.79  & \NMF{MU} \\
 & & 10000.0 & 4.95 & 106.60 & 0.85& \NMF{sp}\\
  & & 4.0 & 6.75 & 133.97 & 0.77 & \NMF{bf} \\[.7ex]  %\hline
 SA & 20 & 3094.0 & 9.47 & 65.67  & 0.00 &\DNMF{ind} \\
  & & 10427.0 & 6.50 & 69.33 & 0.05 & \DNMF{indA}\\
  & & 163.0 & 18.53 & \bfseries 26.44 &  \bfseries -0.37 & \DNMF{dir} \\
  & & 5418.0 & 6.64 & 33.44 & -0.32 & \DNMF{dirA}\\
   & & 3144.0 & 9.47 & 65.69 & 0.00 & \DNMF{comb}\\
  & & 11104.0 & \bfseries 4.17 & 76.83 & 0.14 & \NMF{MU}\\
  & & 3.2 &  21.00 & 30.58 & -0.34 & \NMF{sp}\\
  & & 199.0 &  37.08 & 66.45 & 0.00 & \NMF{bf}\\[.7ex] %\hline
  \ifappendix %% BEGIN if appendix
    LK & 15 & 9999.0 & 3.15  & 64.84 & 0.00  & \DNMF{ind} \\
    & & 9999.0 & 3.05 & 61.30 & 0.06 & \DNMF{indA}\\
  & & 9999.0 & 3.10  & 65.38  &  0.01  & \DNMF{dir} \\
  & & 9999.0 & 3.00 & 65.11 & -0.02 & \DNMF{dirA}\\
  & & 9999.0 & 3.31 & 49.61 & -0.17 & \DNMF{comb}\\
 & & 9999.0 & 2.97  & 99.66  & 0.35  & \NMF{MU} \\
 & & 10000.0 & 3.02 & 99.89 & 0.44 & \NMF{sp}\\
  & & 3.0 & 4.58 & 99.03 & 0.24 & \NMF{bf} \\[.7ex]  %\hline
   HD & 8 & 3773.6 & 7.24 & 50.42  & 0.00 &\DNMF{ind}  \\
    & & 4059.0 & 6.79 & 48.90 & 0.02 & \DNMF{indA}\\
  & & 5103.6 & 6.55 & 29.42 &  -0.12 & \DNMF{dir} \\
 & & 18665.0 & 6.34 & 32.30 & -0.10 & \DNMF{dirA}\\
  & & 6171.0 & 6.96 & 50.05 & -0.00 & \DNMF{comb}\\
 & & 11560.0 & 2.55 & 134.26 & 0.40 & \NMF{MU} \\
  & & 120.4 & 77.48 & 119.86 & 0.47& \NMF{sp} \\
   & & 705.0 & 14.31 & 123.53 & 0.35& \NMF{bf} \\[.7ex] %
 WN & 8 & 6251.0 & 4.29 & 54.01 & 0.00 &\DNMF{ind} \\
  & & 7561.0 & 2.63 & 51.79 & -0.03 & \DNMF{indA}\\
 & & 7579.0 & 4.27 & 24.89 &  0.06 & \DNMF{dir} \\
  & & 10029.7 & 3.59 & 28.02 & -0.16 & \DNMF{dirA}\\
   & & 27444.0 & 0.63 & 120.47 & 0.50 & \NMF{MU}\\
   &  & 83.0 & 50.52 &  107.32 & 0.59 & \NMF{sp} \\
   &  & 28.0 & 10.37 &  131.59 & 0.54 & \NMF{bf} \\[.7ex] %\hline
  \fi %% END if appendix
  \bottomrule
\end{tabular}

==> table_results_supervised.tex <==
\begin{tabular}{@{}
  l% data
  L% k
  S[table-format=5.1,group-minimum-digits=4]% #iters
  S[table-format=2.2]% RE
  S[table-format=3.2]% DE
  S[table-format=+1.2]% ACD
  L% Algorithm
  @{}}
  \toprule
  $\mathcal{D}$ & k & {\#iters} & {$\mathit{RE}$}  &  {$\mathit{DE}$} & {$\mathit{ADC}$} & \text{algorithm}  \\
  \midrule
AB & 2;3 & 11201.0 & 2.53 & 68.54 & 0.00 & \DNMF{ind}  \\
 & & 18174.0 & 2.63 & 71.93 & -0.02 & \DNMF{indA}\\
  & & 3108.1 & 3.00 & 79.49 &  0.00 & \DNMF{dir} \\
  & & 5281.0 & 2.75 & 88.70 & 0.00 & \DNMF{dirA}\\
  & & 9855.0 & 2.79 & \bfseries 66.77 & \bfseries -0.03 & \DNMF{comb}\\
  & &  14287.0 & \bfseries 1.93 & 152.08 &  0.22 & \NMF{MU} \\
  & & 123.7 & 94.14 & 144.56 &  0.14 & \NMF{sp} \\
  & & 834.0 & 21.62 & 161.72 &  0.28 & \NMF{bf} \\
  [.7ex] %\hline
   AR & 7;13 & 2806.0 & 18.74 & 71.27 & 0.00 & \DNMF{ind} \\
    & & 4868.0 & 19.29 & 69.84 & -0.01 & \DNMF{indA}\\
 & &  2286.0 & 17.60 & \bfseries 29.13 &  \bfseries -0.30 & \DNMF{dir} \\
 & & 16788.1 & 17.60 & 30.13 & -0.27 & \DNMF{dirA}\\
 & & 4089.0 & 19.28 & 70.33 & -0.02 & \DNMF{comb}\\
  & & 28318.8 & \bfseries 11.18 & 133.62 & 0.43 & \NMF{MU}\\
 & & 47358.9 & 15.68 & 110.70 & 0.46 & \NMF{sp}\\
 & & 21.0 & 20.45 & 161.60 & 0.35 & \NMF{bf}\\[.7ex]  %\hline
   BRC & 1;2;1;2;1 & 9999.0 & 6.49  & 69.12 & 0.00  & \DNMF{ind} \\
    & & 9999.0 & 6.49 & 65.45 & -0.05 & \DNMF{indA}\\
  & & 9999.0 & 6.48  & 82.68  &  0.05  & \DNMF{dir} \\
  & & 9999.0 & 6.48 & 75.40 & -0.03 & \DNMF{dirA}\\
  & & 9999.0 & 6.51 & \bfseries 60.99 & \bfseries -0.06 & \DNMF{comb}\\
 & & 7953.8 & \bfseries 6.48  & 113.11  & 0.27  & \NMF{MU} \\
 & & 10000.0 & 7.21 & 104.98 & 0.38& \NMF{sp}\\
  & & 17.0 & 7.73 & 97.48 & 0.10 & \NMF{bf} \\[.7ex]  %\hline
   NM & 23;17 & 9999.0 & 8.32  & 66.73 & 0.00  & \DNMF{ind} \\
    & & 9580.4 & 5.16 & 68.39 & 0.15 & \DNMF{indA}\\
  & & 7382.4 & 8.00  & \bfseries 17.18  &  \bfseries -0.32  & \DNMF{dir} \\
  & & 9804.4 & 5.27 & 19.92 & -0.12 & \DNMF{dirA}\\
  & & 9999.0 & 9.46 & 66.98 & -0.02 & \DNMF{comb}\\
 & & 10000.0 & \bfseries 2.53  & 146.56  & 0.38  & \NMF{MU} \\
 & & 10000.0 & 7.01 & 110.13 & 0.43& \NMF{sp}\\
 & & 500.0 & 48.31 & 167.40 & 0.35& \NMF{bf}\\[.7ex]
  \ifappendix %% BEGIN remove from main manuscript
    PD & 3;3 & 9947.8 & 1.47 & 84.46  & 0.00 & \NMF{D} \\
  & & 23061.8 & 1.37 & 58.92 &  -0.34 & \NMF{DE} \\
 & & 50000 & 0.34 & 131.76 & 0.33 & \NMF{MU} \\
  & & 2.1 & 32.60 & 125.42 & 0.06 & \NMF{sp} \\
  & & 41 & 27.92 & 114.78 & 0.09 & \NMF{bf}\\[.7ex]  %\hline
  SE &7;1& 15355.2 & 21.00 & 79.36  &0.00 & \NMF{D} \\
 & & 4460.0 & 13.53 & 39.28 &  -0.33 & \NMF{DE} \\
  & & 10688.0 & 8.60 & 115.47  & 0.21  &  \NMF{MU}\\
  & & 5677.6 & 37.94  & 107.21  & 0.26  & \NMF{sp} \\
  & & 194 & 29.74  & 136.32  & 0.12  & \NMF{bf} \\[.7ex]  %\hline
  \fi %% END remove from main manuscript
  SA & 9;11 & 18761.0 & 4.77 & 73.35 & 0.00 & \DNMF{ind} \\
   & & 10425.0 & 4.56 & 68.41 & -0.02 & \DNMF{indA}\\
  & & 26419.8 & 4.48 & 18.98 &  \bfseries -0.40 & \DNMF{dir} \\
  & & 43839.4 & 3.85 & \bfseries 18.50 & -0.30 & \DNMF{dirA}\\
  & & 16646.0 & 5.12 & 71.90 & -0.01 & \DNMF{comb}\\
  & & 47317.8 & \bfseries 1.69 & 118.95 & 0.32 & \NMF{MU} \\
  & & 50000.0 & 2.61 & 110.06 &0.37 & \NMF{sp}  \\
  & & 49.0 & 29.24 & 110.23 & 0.26 & \NMF{bf}  \\[.7ex]  %\hline
  \ifappendix %% BEGIN remove from main manuscript
  LK & 1;2;1;2;2 & 9999.0 & 3.73  & 67.20 & 0.00  & \DNMF{ind} \\
    & & 9999.0 & 3.72 & 63.84 & -0.03 & \DNMF{indA}\\
  & & 9999.0 & 3.72  & 89.68  &  0.09  & \DNMF{dir} \\
  & & 9999.0 & 3.71 & 85.10 & 0.08 & \DNMF{dirA}\\
  & & 9999.0 & 3.76 & 54.85 & -0.15 & \DNMF{comb}\\
 & & 9830.8 & 3.71  & 128.86  & 0.37  & \NMF{MU} \\
 & & 207.2 & 23.88 & 109.25 & 0.49& \NMF{sp}\\
  & & 7.0 & 4.84 & 140.16 & 0.38 & \NMF{bf} \\[.7ex]  %\hline
  BC & 2;6 &15793.4 & 2.52 & 66.54 & 0.00 & \NMF{D} \\
  & & 47023.8 & 2.54 & 18.29 &  -0.35 & \NMF{DE} \\
 & & 26388.6 & 0.21 & 119.12 & 0.29  & \NMF{MU} \\
  & & 35182.5 & 2.28 & 106.79 & 0.41 & \NMF{sp} \\
  & & 70.0 & 24.46 & 123.99 & 0.36 & \NMF{bf} \\[.7ex]  %\hline
 HD & 6;2 & 16318.0 & 4.92 & 63.24 & 0.00 & \DNMF{ind} \\
     & & 37556.6 & 3.26 & 61.97 & 0.00 & \DNMF{indA}\\
  & & 21214.0 & 4.95 & 20.17 &  -0.17 & \DNMF{dir} \\
  & & 43258.6 & 5.26 & 20.77 & -0.23 & \DNMF{dirA}\\
 	& & 19056.0 & 5.78 & 64.07 & -0.04 & \DNMF{comb}\\
 & & 32516.0 & 0.42 & 140.06  & 0.21 & \NMF{MU} \\
  & & 136.9 & 64.77  &  116.02  & 0.31 & \NMF{sp}\\
  & & 528.0 & 14.28  &  137.32  & 0.23 & \NMF{bf}\\[.7ex]  %\hline ->here
  WN & 3;1;2 & 20796.0 & 2.68 & 56.75 & 0.00 & \NMF{D} \\
 & &  28673.7 & 2.34 & 16.08 &  -0.20 & \NMF{DE} \\
 & & 27466.0 & 0.64 & 106.17 & 0.33 &  \NMF{MU}\\
 & & 34553.4 & 4.05 & 103.16  & 0.49 & \NMF{sp} \\
 & & 28 & 10.37 & 119.21  & 0.36 & \NMF{bf} \\
  \fi %% END remove from main manuscript
  \bottomrule
 \end{tabular} 
